Tactile Ergodic Coverage on Curved Surfaces

In this article, we present a feedback control method for tactile coverage tasks, such as cleaning or surface inspection. These tasks are challenging to plan due to complex continuous physical interactions. In these tasks, the coverage target and progress can be easily measured using a camera and encoded in a point cloud. We propose an ergodic coverage method that operates directly on point clouds, guiding the robot to spend more time on regions requiring more coverage. For robot control and contact behavior, we use geometric algebra to formulate a task-space impedance controller that tracks a line while simultaneously exerting a desired force along that line. We evaluate the performance of our method in kinematic simulations and demonstrate its applicability in real-world experiments on kitchenware. Our source codes, experimental data, and videos are available as open access at https://sites.google.com/view/tactile-ergodic-control/

==> floats/boxplot_alpha.tex <==
\begin{figure}[ht]
        % % % %
        \centering
        % % % % 
        \includegraphics[width=1.0\linewidth]{floats/boxplot_alpha1.pdf}
        % % % % 
        \caption{Exploration performance measured by the normalized ergodic metric \eqref{eq:ergodicity} with respect to the diffusion scalar $\alpha$ in \eqref{eq:timestep}}
        % % % %
        \label{fig:box_plot_alpha}
\end{figure}

==> floats/boxplot_nb_eigen.tex <==
\begin{figure}[ht]
        % % % %
        \centering
        % % % % 
        \includegraphics[width=1.0\linewidth]{floats/boxplot_nb_eigen1.pdf}
        % % % % 
        \caption{Exploration performance measured by the normalized ergodic metric $\epsilon_t$ \eqref{eq:ergodicity} with respect to the number of eigencomponents $\neigen$ used in the spectral formulation \eqref{eq:spectral_diffusion}.}
        % % % %
        \label{fig:box_plot_nb_eigen}
\end{figure}

==> floats/complexity_table.tex <==
\begin{table}[htbp]
    \centering
    \caption{Computation time required for computing the discrete Laplacian $\bm{L}$ and the mass matrix $\bm{M}$ using the \emph{robust\_laplacian} package}
    \label{tab:performance}
    % \tabcolsep=0.11cm
    \small
    \begin{tabular}{ccccccc}
        \toprule
        $n_{\mathcal{P}}$ & 2996 & 6070 & 9097 & 11910 & 14993 & 18001 \\
        \midrule
        Time [ms] & 59 & 103 & 178 & 228 & 293 & 342 \\
        \bottomrule
    \end{tabular}
\end{table}



==> floats/parameters.tex <==
\begin{table}[htbp]
    \centering
    \caption{Fixed parameters used in the experiments.}
    \label{tab:parameters}
    % \tabcolsep=0.11cm
    \small
    \begin{tabular}{cccccc}
        \toprule
        Parameters & $\ddot{\bm{x}}_{max}$ & $\dot{\bm{x}}_{max}$ &   Voxel size\\
        \midrule
        Values & 3 [$mm/s^2$] & 3 [$mm/s$] & 3 [$mm$] \\
        \bottomrule
    \end{tabular}
\end{table}

==> floats/runtime_flow.tex <==
\begin{algorithm}
            \SetKwBlock{y}{}{}
            \KwIn{$\mathcal{T}, \bm{q}, M, \tilde{\bm{c}} (\bm{x}, t)$}
            \KwOut{$P_a'$, $X$, $P_i$, $\bm{c}( \bm{x},t)$}
     
        Solve forward kinematics \eqref{} $P_a$ using \eqref{eq:}
        compute local neighborhood using $P_a$
        initialize agents and bodies using using \eqref{eq:fkin} and $\bm{q}_0$
        
        compute $\delta t$ using \eqref{eq:cfl}
        
{
        \While{true} 
        {
            compute $c(\bm{x},t)$ and $s(\bm{x},t)$ as in \cite{ivicErgodicityBasedCooperativeMultiagent2017}

            
            \For{$k \gets 1$ to $N_k$}{
                integrate \eqref{eq:heat} using \eqref{eq:integration}
            }
            

            \For{all $M$ bodies}{


            \For{all $N_j$ agents}{
                        compute $\bm{x}_{i,j}$ and $\bm{f}_{i,j}$ using \eqref{eq:fkin} and \eqref{eq:force}
                }   
                
                compute $\bm{v}_{\text{des}_j}$ and $w_j$ using \eqref{eq:twist} and \eqref{eq:link_weight}
            }
           

            compute $\dot{\bm{q}}_{\text{des}}$ using  \eqref{eq:q_des}}}
      

        \caption{Tangent Space and Coverage Computation}
        \label{alg:main_loop}
    \end{algorithm}
